EXAMS: A Multi-Subject High School Examinations Dataset for Cross-Lingual and Multilingual Question Answering

We propose EXAMS -- a new benchmark dataset for cross-lingual and multilingual question answering for high school examinations. We collected more than 24,000 high-quality high school exam questions in 16 languages, covering 8 language families and 24 school subjects from Natural Sciences and Social Sciences, among others. EXAMS offers a fine-grained evaluation framework across multiple languages and subjects, which allows precise analysis and comparison of various models. We perform various experiments with existing top-performing multilingual pre-trained models and we show that EXAMS offers multiple challenges that require multilingual knowledge and reasoning in multiple domains. We hope that EXAMS will enable researchers to explore challenging reasoning and knowledge transfer methods and pre-trained models for school question answering in various languages which was not possible before. The data, code, pre-trained models, and evaluation are available at https://github.com/mhardalov/exams-qa.

==> sections/summary.tex <==

\paragraph{Contributions/Summary:}

\begin{enumerate}[noitemsep]
    \item New Dataset from Multilingual (Multiple-choice) School Questions;
    \item 16 Different languages from 8 language families; See Table~\ref{tab:langquestionstats};
    \item Fine-grained per-subject evaluation (3 types of Questions -- Natural Science, Social Science, Other);
    Total of 16+ Subjects;
    See Figure~\ref{fig:subject_dist}.
    \item Parallel data between some of the languages:
        \begin{itemize}
            \item Croatia: Croatian, Serbian, Italian, Hungarian (1000+, except Hungarian)
            \item Hungary: German, French, Spanish, Croatian, Italian, Serbian, Croatian (not so much up to 600)
            \item N. Macedonia: Macedonian, Albanian, Turkish (1000+ per language)
        \end{itemize}{}
    \item Around 500-700 questions from 8th (or lower) grade + 400 (online quizzes in Bulgarian) in Arabic and Bulgarian,
    which can be used as an ''Easy'' set;
    \item Built a corpus from Wikipedia articles for each language to obtain context paragraphs;
    \item Evaluated mandatory baselines and some interesting experiments (See Section~\ref{sec:models}:
    \begin{itemize}
        \item (Mandatory) Random guess ;
        \item (Good-to-have) Information retrieval ranker using Wikipedia as a corpus;
        \item (Mandatory) Fine-tuned state-of-the-art multilingual models (mBERT, XLM-R, XLM-R-Large) on several English datasets (RACE, ARC-Easy, ARC-Challenge).
        \item (BERTology) The latter but with some layers frozen (Embeddings, the first N layers) (BERTology).
        \item (BERTology) BERT as Knowledge-base. Ranking using the knowledge in the LM (using [MASK]ing).
        \item (Nice-to-have) Do multilingual data help? One-vs-all (language/family) additional fine-tuning, and evaluation using examples from our dataset. (Not done yet.)
    \end{itemize}{}
\end{enumerate}{}

\paragraph{What is our focus:}
\begin{enumerate}[noitemsep]
    \item The newly collected dataset;
    \item The BERTology experiments;
    \item Error Analysis:
    \begin{itemize}
        \item Which subjects are harder, and why?
        \item Is the shortcomings in IR model and the size of Wikipedia correlate with lower scores?
        \item Analyze some real examples.
    \end{itemize}
    

    
    \item Why is our dataset better, or different than the rest, and why it is important: 
    \begin{itemize}
        \item New and diverse languages;
        \item Parallel data;
        \item Fairly large ~24,000 questions;
        \item Created by professionals (official exams), not turks;
        \item Complex reasoning in some categories, hard questions overall (for 12th graders);
        \item There are a lot of monolingual multiple-choice datasets but none of them is multilingual.
    \end{itemize}
    \item We open a new direction the exact one that ARC opened several years ago, and is still not solved! 
\end{enumerate}{}
